Mapping and Cleaning Open Commonsense Knowledge Bases with Generative Translation

Structured knowledge bases (KBs) are the backbone of many know\-ledge-intensive applications, and their automated construction has received considerable attention. In particular, open information extraction (OpenIE) is often used to induce structure from a text. However, although it allows high recall, the extracted knowledge tends to inherit noise from the sources and the OpenIE algorithm. Besides, OpenIE tuples contain an open-ended, non-canonicalized set of relations, making the extracted knowledge's downstream exploitation harder. In this paper, we study the problem of mapping an open KB into the fixed schema of an existing KB, specifically for the case of commonsense knowledge. We propose approaching the problem by generative translation, i.e., by training a language model to generate fixed-schema assertions from open ones. Experiments show that this approach occupies a sweet spot between traditional manual, rule-based, or classification-based canonicalization and purely generative KB construction like COMET. Moreover, it produces higher mapping accuracy than the former while avoiding the association-based noise of the latter.

==> parts/discussions.tex <==
\section{Discussions}
This is a discussion.
\todo[inline]{Generalization to other contexts}

\todo[inline]{Here, it looks more like RP rather than NP canonicalization.}

\todo[inline]{More complex models.}

==> parts/existing_systems_long.tex <==
\subsection{Existing Systems}

OpenKI~\cite{zhang2019openki} considered the task of predicting what would the predicate of an open triple \textit{(s, p, o)} be in a CloseKB. This is basically a classification task where the classifier needs to predict $p'$ a predicate in a CloseKB such that \textit{(s, p', o)} is semantically equivalent/related to \textit{(s, p, o)}. The main idea of the algorithm is to encode an entity using its neighbor relations (themselves encoded with embeddings that are learned from scratch). This way, the authors claim the algorithm should be able to generalize. However, this approach suffers several problems.
First, the approach generalizes to unseen entities but not to unseen relations. With OpenKBs, this is a significant issue as predicates are very sparse, and it is very likely that many of them were not even observed during training. This problem was partially solved by~\cite{wood2021integrating} by using a language model to compute embeddings for each predicate and then combine this representation with a learned embedding. This last parameter will not be learned if we did not see the predicate.
Second, the training and testing dataset is constructed using an OpenKB and a CloseKB with entities already aligned by humans (ReVerb~\cite{fader2011identifying} and Freebase in the original paper). However, this is not generally the case in practice. Besides, it considers that the subject and object remain the same (thus ignoring modification of the subject and object, inverse relations, or closely related entities).
Third, the neighborhood used to encode the relations comes from both the OpenKB and the CloseKB. That makes the model learn to select one of the relations in the CloseKB in the neighborhood of both the subject and the object and to predict it (in the dataset provided by the authors, the relation to predict is indeed in the input, among the other relations). However, this is not the case in practice, where we have many subject-object pairs in the OpenKB that have no connection in the CloseKB.
Finally, the approach is evaluated according to a single metric, the Mean Average Precision (MAP). Unfortunately, this metric fails to measure how well the approach generalizes on unseen entities, predicates, or statements (the CloseKB is never complete).

Many systems tried to use manual rules or mine them to do the mapping. In~\cite{soderland2013open}, the authors use manual rules that can describe a few semantic information (like the type of elements in the open triples). However, they require much human work and fail to scale to large knowledge bases. In~\cite{soderland2010adapting}, the authors first detect entity types in the subjects and objects using regular expressions. Then, they use rule mining on the types and keywords in the triple to do the mapping. For each rule, they compute a confidence score. This approach has several problems. First, we need to be able to classify (by type) the subjects and objects, which is not the case here. Second, the classification is done by hand. Third, the rules poorly generalize to unseen entities and predicates. In~\cite{dutta2014semantifying}, the authors mine association rules between an open predicate and a predefined predicate over a particular domain. They start by performing entity linking, and then they align triples from the OpenKB (NELL) and the CloseKB (DBpedia). Like for OpenKI, the approach does not generalize to sparse or unseen predicates. Therefore, it requires a considerable overlap between the OpenKB and the CloseKB, which is not the case here. Besides, we have the constraint that the subject and the object must match in both KBs to have an alignment.

KBPearl~\cite{lin2020kbpearl} is a system for performing knowledge base population: Given an incomplete KB and a document, their goal is to complete the KB using the information in the document. First, the system extracts open triples and side information (that we do not have in our case) from the document. Then, it performs simple canonicalization over the entities and predicates. Next, it maps jointly the noun phrases (representing the subjects and the objects) and the relational phrases from the OpenKB to entities and predicates in the CloseKB. The primary constraint here is that the mapping between a noun phrase (resp. a relational phrase) and an entity (resp. a predicate) only happens if the relational phrase is already a known label for the entity (resp. the predicate). This is very restrictive in practice as we might have few or no labels for the entities and predicates (none in the case of ConceptNet), making the linking to related entities impossible.

In~\cite{putri2019aligning}, the authors propose a method to compute the similarity between a triple in an OpenKB and a triple in a CloseKB. This differs from our approach in which we do not know in advance potential candidates in the CloseKB. Indeed, the CloseKB is often incomplete, and we want to generate new triples thanks to the OpenKB. Therefore, we focus more on the generation rather than the comparison. However, it is essential to notice that this approach integrates word embeddings for the comparison. Besides, the authors use the distant supervision approach to create a dataset automatically: Given a close triple, they find sentences (in an additional corpus) containing both entities from the triple. Then, they apply an OpenIE algorithm to obtain an open triple. This triple is used as a ground truth. In our case, we do not have this additional textual source: The inputs are the OpenKB and the CloseKB.

In~\cite{gashteovski2020aligning}, the authors introduce a methodology to manually evaluate the alignment of triples from an OpenKB with a CloseKB. Besides, they studied how much an OpenKB (OPIEC~\cite{gashteovski2019opiec} in their case) can be expressed by a CloseKB (DBpedia~\cite{auer2007dbpedia}). They found that the open triples can often be aligned to DBpedia facts, but they are generally more specific. Besides, one can generally express an OpenIE fact in the DBpedia schema, but this expressivity is limited if we consider only a single relation rather than a logic formula.

==> parts/introduction-old.tex <==
\section{Introduction}
\label{sec:introduction}

\paragraph{Motivation and Problem}
Open Information (OpenIE) automatically extracts knowledge from a textual data source. The idea is to find explicit relationships in the text together with the subject and the object they link. For example, from the sentence ``In nature, fish swim freely in the ocean.'', OpenIE could extract the triple \textit{(fish, swim in, the ocean)}. Here, the text explicitly mentions the subject, the predicate, and the object. Therefore, if we use OpenIE to construct a knowledge base (we call it an Open Knowledge Base, open KB) from many sentences, we will obtain data with little structure, many predicates, redundant statements, and ambiguity.

OpenIE is often used for commonsense knowledge base (CSKB) construction. Previous works such as TupleKB~\cite{mishra2017domain}, Quasimodo~\cite{quasimodo,10.1145/3340531.3417416} or Ascent~\cite{nguyen2021refined,nguyen2021advanced,nguyen2021inside} use OpenIE to extract knowledge from different textual sources (textbooks, query logs, question-answering forums, search engines, or the Web) and then add additional steps to clean and normalize the obtained data. Another example is ReVerb~\cite{fader2011identifying}, which was used to obtain OpenIE triples from a Web crawl. The output of OpenIE typically inherits noise from sources and extraction, and the resulting knowledge bases contain an open-ended set of predicates. This is typically not the case for knowledge bases with a predefined schema. Popular instances of this type are manually constructed, like ConceptNet~\cite{conceptnet} and ATOMIC~\cite{comet-atomic-2020}. Therefore, they tend to have higher precision. Besides, they are frequently used in downstream applications such as question-answering \cite{mhgrn,yasunaga2021qagnn}, knowledge-enhanced text generation~\cite{10.1145/3512467}, image classification~\cite{DBLP:conf/aaai/WangHLLZMW20}, conversation recommender systems~\cite{DBLP:conf/kdd/ZhouZBZWY20}, or emotion detection~\cite{zhong-etal-2019-knowledge}. These applications assume there are few known predicates so that we can learn specialized parameters for each relation (a matrix or embeddings with a graph neural network). This is not the case for open KBs.

Still, many properties of open KBs, such as high recall and ease of construction, are desirable. In this paper, we study \textit{how to transform an open KB into a knowledge base with a predefined schema}. More specifically, we study the case of commonsense knowledge, where ConceptNet is by far the most popular resource. From an open KB, we want to generate a knowledge base that has the same relation names as ConceptNet. This way, we aim to increase the precision and rank the statements better, while keeping the high recall of OpenIE. Specifically, as we reduce the number of relations, we might be able to make the statements corroborate. For example, \textit{(fish, live in, water, freq:1)}, \textit{(fish, swim in, water, freq:1)} and \textit{(fish, breath in, water, freq:1)} can be transformed into \textit{(fish, LocatedIn, water, freq:3)} in ConceptNet, and therefore they all help to consolidate that statement. Besides, we will make new knowledge bases available to work with many existing applications originally developed for ConceptNet.

Transforming open triples to a predefined schema raises many challenges. In the simplest case, the subject and the object are conserved, and we only need to predict the correct predefined predicate. This would be a classification task. For example, \textit{(fish, live in, water)} can be mapped to \textit{(fish, LocatedAt, water)} in ConceptNet. We could proceed similarly in the case where the subject and the object are inverted, like in \textit{(ocean, contain, fish)} that can be mapped to \textit{(fish, LocatedAt, ocean)}. So, we additionally need to consider inverting relations. However, in many cases, the object is not even expressed in the same way or only partially: \textit{(fish, live in, the ocean)} can be mapped to \textit{(fish, LocatedAt, ocean)}. In other cases, part or all of the predicate is in the object, like in \textit{(fish, swim in, the ocean)} that can be mapped to \textit{(fish, CapableOf, swim in the ocean)}. Here, the initial triple could also be mapped to \textit{(fish, LocatedAt, ocean)}, showing that the mapping is not always unique. Other problems might also arise, like with (near) synonyms. For example, we might want to map \textit{(fish, live in, sea)} with \textit{(fish, LocatedAt, ocean)}.

\paragraph{Approach and Contribution}
In this paper, we propose to approach the mapping of an open KB to a predefined set of relations as a translation task. We start by aligning triples automatically from the source KB with triples from the target KB. Then, we use this dataset to finetune a generative language model (LM) to generate the translations: Given as input a triple from an open KB, our model can turn it into one or several triples in the target KB. The generative nature of the LM allows it to adapt to the abovementioned problems while keeping a high faithfulness w.r.t.\ the source KB. Besides, we show that this improves the precision of the original KB and provides a better ranking for the statements while still keeping a high recall.

We first introduce previous works in Section~\ref{sec:previous_work}. Then, we define our problem formally in Section~\ref{sec:problem}. In Section~\ref{sec:model}, we present our methodology with the model we use and how we construct a dataset automatically. In Section~\ref{sec:experiment_setup}, we describe the setup of our experiments. In Section~\ref{sec:experiments}, we compare the models and see the advantages of using an LM-based translation model. Our contributions are the following:

\begin{enumerate}
    \item We define the problem of open KB mapping, delineating it from the more generic canonicalization and the more specific predicate classification problems.
    \item We propose a generative translation model based on pre-trained language models and automatically constructed training data.
    \item We experimentally verify the advantages of this method compared to traditional manual and rule-based mapping, classification, and purely generative methods like COMET.
\end{enumerate}



==> parts/old/detailled_previous_works.tex <==
In~\cite{gashteovski2020aligning}, the authors introduce a methodology to manually evaluate the alignment of triples from an OpenKB with a CloseKB. Besides, they studied how much an OpenKB (OPIEC~\cite{gashteovski2019opiec} in their case) can be expressed by a CloseKB (DBpedia~\cite{auer2007dbpedia}). They found that the open triples can often be aligned to DBpedia facts, but they are generally more specific. Besides, one can generally express an OpenIE fact in DBpedia schema, but this expressivity is limited if we consider only a single relation rather than a logic formula.

OpenKI~\cite{zhang2019openki} considered the task of predicting what would the predicate of an open triple \textit{(s, p, o)} be in a CloseKB. This is basically a classification task where the classifier needs to predict $p'$ a predicate in a CloseKB such that \textit{(s, p', o)} is semantically equivalent/related to \textit{(s, p, o)}. The main idea of the algorithm is to encode an entity using its neighbor relations (themselves encoded with embeddings that are learnt from scratch). This way, the author claim the algorithm should be able to generalize. However, this approach suffers several problems.
First, the approach generalized to unseen entities but not to unseen relations. With OpenKBs, this is a major issue as predicates are very sparse and it is very likely that many of them where not even observed during training. This problem was partially solved by~\cite{wood2021integrating} by using a language model to compute embeddings for each predicate and then combine this representation with a learnt embedding. This last parameter will not be learnt if we did not see the predicate.
Second, the training and testing dataset is constructed using an OpenKB and a CloseKB with entities already aligned (ReVerb~\cite{fader2011identifying} and Freebase in the original paper). This is not generally the case in practice, it considers that the subject and object remain the same (thus ignoring inverse relations or closely related entities) and it limits the size of the dataset we can create (see the points mentioned earlier about the difficulties during the alignment).
Third, the neighborhood used to encode the relations comes from both the OpenKB and the CloseKB. That makes the model learn to select one of the close relation in the neighborhood of both the subject and the object and to predict it (in the dataset provided by the authors, the relation to predict is indeed in the input, among the other relations). This is not the case in practice where we have many subject-object pairs in the OpenKB that have no connection in the CloseKB.
Finally, the approach is evaluated according to a single metric, the Mean Average Precision (MAP). This metric fails to measure how well the approach generalizes on unseen entities, predicates or statements (the CloseKB is never complete).

~\cite{dutta2013integrating} focuses on entity linking between an OpenKB (NELL and ReVerb) and a CloseKB (DBpedia). It does not consider predicate and triple mapping.


% Rule mining/Manual rules
In~\cite{soderland2013open} the authors turn open triples into close triples using a set of rules. These rules allow to describe a few semantic information (like the type of elements in the open triples), but they require a lot of human work and fail to scale to large knowledge bases.

In~\cite{soderland2010adapting}, the authors first detect entity types in the subjects and objects using regular expressions. Then, they use rule mining on the types and keywords in the triple to do the mapping. For each rule, they compute a confidence score. This approach has several problems. First, we need to be able to classify the subjects and objects, which is not the case in our case. Second, the classification is done by hand. Third, the rules poorly generalize to unseen entities and predicates.

In~\cite{dutta2014semantifying}, the authors mine association rules between an open predicate and a predefined predicate over a certain domain. They start by performing entity linking and then they align triples from the OpenKB (NELL) and the CloseKB (DBpedia). Like for OpenKI, the approach does not generalize to sparse or unseen predicates. Therefore, it requires a large overlap between the OpenKB and the CloseKB, which is not the case for us here. Besides, we have the constraint that the subject and the object must match in both KBs to have an alignment.


HARPY~\cite{grycner2014harpy} is a system based on random walks in a graph that aligns relational phrases in Patty~\cite{nakashole2012patty} with verb senses in WordNet~\cite{miller1995wordnet}. This setting differs from the one we target: We do not have knowledge bases and Patty comes with annotations such as the type of the arguments of a predicate and hypernymity information between predicates.

KBPearl~\cite{lin2020kbpearl} is a system for performing knowledge base population: Given an incomplete KB and a document, their goal is to complete the KB using the information in the document. The system extracts open triples and side information (that we do not have in our case) from the document. Then, it performs a simple canonicalization over the entities and predicates. Next it maps jointly the noun phrases (representing the subjects and the objects) and the relational phrases from the OpenKB to entities and predicates in the CloseKB. The main constraint here is that the mapping between a noun phrase (resp. a relational phrase) and an entity (resp. a predicate) only happens if the relational phrase is already a known label for the entity (resp. the predicate). This is very restrictive in practice as we might have few or no labels for the entities and predicates (none in the case of ConceptNet), and it makes the linking to related entities impossible.

In~\cite{putri2019aligning}, the authors propose a method to compute the similarity between a triple in an OpenKB and a triple in a CloseKB. This differs from our approach in which we do not know in advance potential candidates in the CloseKB. Indeed, the CloseKB is often incomplete and we want to generate new triples thanks to the OpenKB. Therefore, we focus more on the generation rather than the comparison. However, it is important to notice that this approach integrates word embeddings for the comparison. Besides, the author use the distant supervision approach to automatically create a dataset: Given an close triple, they find sentences (in an additional corpus) containing the both entities from the triple and then they apply an OpenIE algorithm to obtain an open triple. This triple is used as a ground truth. In our case, we do not have this additional textual source: The inputs are the OpenKB and the CloseKB.


==> parts/old/preliminaries.tex <==
\section{Preliminaries}

\paragraph{Open Knowledge Base} An open knowledge base (OpenKB) is a collection of SPO triples \textit{(Subject, Predicate, Object)} such that there is no constraint on all the components. It means that they are not canonicalized. For example, the triples \textit{(The Statue of Liberty, is in, New York)} and \textit{(Statue of Liberty, located in, NYC)}, although equivalent, could be present in the same knowledge base. In general, both the subject and the object are noun phrases (NP), whereas the predicate is a relational phrase (RP). As a comparison, knowledge bases with a predefined schema like Wikidata~\cite{vrandevcic2014wikidata}, YAGO~\cite{tanon2020yago} or ConceptNet~\cite{conceptnet} come with a set of predefined predicates and/or entities for the subjects and the objects. This paper will call such a knowledge base a Close Knowledge Base (CloseKB).

\paragraph{Construction of OpenKBs} The construction of OpenKBs relies on Open Information Extraction (OpenIE) algorithms. These algorithms take as input a text and return a set of open triples such that the subject, the predicate, and the object are explicitly mentioned in the text. There exist several systems like CoreNLP~\cite{manning2014stanford} or OpenIE6~\cite{kolluru2020openie6}.

\paragraph{Open Knowledge Base Canonicalization} The task of OpenKB canonicalization consists of turning an open triple \textit{(s, p, o)}, where s and o are an NP and p is a RP, into an equivalent (semantically) new triple \textit{($s_e$, $p_e$, $o_e$)}, where $s_e$ and $o_e$ represent entities (generally through a non-ambiguous NP) and $p_e$ is a non-ambiguous and unique representation of a predicate. It means there is no other $p_e'$ such that \textit{($s_e$, $p_e$, $o_e$)} is semantically equivalent to \textit{($s_e$, $p_e'$, $o_e$)}. For example, we would like to map \textit{(Statue of Liberty, located in, NYC)} to \textit{(The Statue of Liberty, AtLocation, New York City)}, where ``The Statue of Liberty'' represents only the famous monument in New York City, ``New York City'' represents unambiguously the American city, and ``AtLocation'' is a predicate used to give the location of the subject.  

NP canonicalization is more studied than RP canonicalization, but the task is generally treated as a clusterization problem~\cite{galarraga2014canonicalizing}. It is important to notice that an NP or an RP does not necessarily belong to a single cluster as this cluster may depend on the context. For example, in \textit{(Obama, be, president of the US)}, ``Obama'' refers to the entity ``Barack Obama'', whereas in \textit{(Obama, wrote, Becoming)}, ``Obama'' refers to ``Michele Obama''. Also, we must notice that the canonicalization does not have a target: The transformation does not try to imitate the schema of an existing knowledge base. The main goal here is to reduce redundancy, but the number of predicates might remain high. In our scenario, we aim for a predifined set of relations.

\paragraph{Entity Linking} Entity Linking is a task that consists in mapping an entity name to an entity in a knowledge base. For example, we would like to map \textit{Paris} in \textit{(Paris, be, city of love)} to \href{https://www.wikidata.org/wiki/Q90}{Q90} in Wikidata, the entity that represents the capital of France. In the triple \textit{(Paris, be, a hero)}, \textit{Paris} should be mapped to \href{https://www.wikidata.org/wiki/Q167646}{Q167646} in Wikidata, the entity that represents the son of Priam. When mapping an OpenKB to a CloseKB, most systems first perform entity linking before processing the predicate~\cite{dutta2014semantifying,zhang2019openki}. This supposes that subject and the object remain unchanged during the mapping. This is a problem when we want to map to ConceptNet as this KB is not canonicalized and the subject and object might be modified.

\paragraph{Knowledge Base Alignment} The task of KB alignment is composed of two sub-tasks: Entity alignment and predicate alignment. Entity alignment is the most common. It consists of mapping entities from a first knowledge base to an equivalent entity in a second KB. Predicate alignment works the same way: We want to map predicates from a given KB to equivalent predicates in another one. The problem when we work with OpenKBs is that we do not work with unique representations but with NPs and RPs. Therefore, the alignment must happen at the level of each triple. Let's say we want to align an OpenKB $\mathcal{K}_O$ with a CloseKB $\mathcal{K}_C$. Given a triple \textit{(s, p, o)} in $\mathcal{K}_O$, we want to align it to a semantically equivalent triple \textit{($s_e$, $p_e$, $o_e$)} in $\mathcal{K}_C$. As OpenKB are generally more expressive and such an equivalent representation might not exist, we can relax the alignment by only requiring a semantic closeness. For example, \textit{(fish, swim in, ocean)} could be align with \textit{(fish, LocatedIn, ocean)} if the CloseKB does not contain a predicate for swimming. If we consider scored triples, the fact that several triples might lead to the same alignment means that we can perform corroboration to rerank the statements and potentially increase the precision.

\paragraph{Knowledge Base Construction} The task of knowledge base construction consists of building a knowledge base. This can be done manually by asking humans to fill in the KB or automatically using pattern matching of OpenIE. In both cases, the goal is to improve precision and recall. In general, manual approaches have higher accuracy but fail to scale. In our case, translating an OpenKB to a CloseKB can be seen as an additional stage in an OpenIE extraction pipeline. By doing so, we make our KB match a predefined schema.


==> parts/rule_mining.tex <==
\subsubsection{Rule Mining}

Given that no previous work made their implementation public, we propose a rule mining approach inspired by previous works~\cite{soderland2013open,soderland2010adapting,dutta2014semantifying}. Our method requires a training dataset of mappings. In our case, this dataset was constructed automatically (see Section~\ref{sec:alignment}) using the rule-based alignment method. The LM-based alignment is inappropriate as the subject and object must remain unchanged with the rule mining approach. Like in previous works, we also used WordNet to get the type of the concepts.

We use AMIE~\cite{lajus2020fast} to mine Horn rules of the form $B \Rightarrow r(x, y)$. The PCA confidence proposed in AMIE yields poor results. Therefore, we used the standard confidence. Ultimately, we only keep rules with a confidence score greater than 0.5. An advantage of this method is that it provides high interpretability: For each final generation, we can see which open triples were used to generate it and which rules were applied.

==> parts/tables/auto_rec_prec.tex <==
\begin{table*}[!ht]
    \centering

\begin{adjustbox}{width=\textwidth,center}
\begin{tabular}{|c|c|c|c|c|c|c|HHHc|c|c|c|c|}
        \textbf{KB}  & \textbf{Method} & \textbf{Training data} & $R_a$ & $\overline{R_a}$ & $P_a$ & $\overline{P_a}$ & $P_a@10$ & $P_a@100$ & $P_a@1000$ & $P_a@10k$ & $\overline{P_a}@10k$ & MRR & $\overline{MRR}$ & \textbf{Size} \\
        \hline \hline
        ConceptNet & KB itself & - & - & - & - & - & - & - & - & - & -  & - & - & 232,532 \\
        \hdashline
        Quasimodo & KB itself & - & 2.54\%$^*$ & - & 0.271\%$^*$ & - & 10\%$^*$ & 17\%$^*$ & 11\%$^*$ & 4.79\%$^*$ & -  & 4.63$e^{-6}$ $^*$ & - & 5,930,628\\
        \hdashline
        Ascent++ & KB itself & - & 1.63\%$^*$ & 1.63\%$^*$ & 0.430\%$^*$ & - & 10\%$^*$ & 10\%$^*$ & 6.6\%$^*$ & 3.13\%$^*$ & - & 3.56$e^{-6}$ $^*$  & - & 1,967,126\\
        \hline
        \multirow{8}{*}{Quasimodo} & Manual Mapping~\cite{nguyen2021refined} & - & 0.588\% & - & 2.78$e^{-2}$\% & - & 10\% & 8\% & 5\% & 1.51\% & - & 2.74$e^{-6}$ & - & 4,925,792 \\
         & Rule Mining~\cite{soderland2013open,soderland2010adapting,dutta2014semantifying} & Rule-based & 0.409\% & 1.60$e^{-2}$\% & 0.138\% & 5.37$e^{-3}$\% & 30\% & 21\% & 7.1\% & 1.75\% & 2.04$e^{-2}$\% & $5.83e^{-6}$ & 7.69$e^{-9}$ & 689,146 \\
         & Classifier~\cite{zhang2019openki} & Rule-based & 1.91\% & 0.106\% & 8.11$e^{-2}$\% & 4.42$e^{-3}$\% & 20\% & 17\% & 9.4\% & 3.22\% & 1.04$e^{-2}$\% & $6.57e^{-6}$ & 4.87$e^{-9}$ & 5,478,028 \\
        \hdashline
         & GenT@1 & Rule-based & 3.72\% & 1.08\% & \textbf{0.209\%} & 5.89$e^{-2}$\% & 80\% & 76\% & 45.4\% & 16.1\% & 0.961\% & $2.23e^{-5}$ & 4.52$e^{-7}$ & 4,135,349 \\
         & GenT@10 & Rule-based & 6.51\% & 3.35\% & 4.78$e^{-2}$\% & 2.29$e^{-2}$\% & \textbf{90\%} & \textbf{78\% }& \textbf{46.5\%} & \textbf{17.3\%} & 1.12\% & \textbf{2.30}$e^{-5}$  & 4.51$e^{-7}$ & 33,425,732 \\
        \hdashline
         %& LM-based@1 & LM-based@0.1 & 1.38\% & 1.03\% & 0.131\% & 9.71$e^{-2}$\% & 60\% & 39\% & 14.3\% & 4.37\% & 1.37\% & 1.21$e^{-5}$  & 4.72$e^{-7}$ & 2,458,687 \\
         %& LM-based@10 & LM-based@0.1 & 2.90\% & 2.49\% & 3.29$e^{-2}$\% & 2.81$e^{-2}$\% & 60\% & 38\% & 14.8\% & 4.32\% & 1.23\% & 1.28$e^{-5}$ & 4.79$e^{-7}$& 20,738,235  \\
         %& LM-based@1 & LM-based@1 & 3.38\% & 1.85\% & 0.472\% & 2.55$e^{-1}$\% & 30\% & 39\% & 34.5\% & 13.7\% & 2.21\% & 1.08$e^{-5}$  & 3.45$e^{-7}$ & 1,669,647\\
         & GenT@10 & LM-based@10k & 6.02\% & 4.26\% & 9.40$e^{-2}$\% & \textbf{6.38$e^{-2}$\%} & 20\% & 39\% & 35.5\% & 13.3\% & 1.71\% & 1.16$e^{-5}$ & 3.21$e^{-7}$ & 15,647,853 \\
         %& LM-based@1 & LM-based@10 & 6.47\% & 1.04\% & \textbf{2.28\%} & \textbf{3.65$e^{-1}$}\% & 20\% & 40\% & 40.8\% & \textbf{34.5\%} & 0.981\% & 1.35$e^{-5}$ & 1.09$e^{-7}$ & 659,120 \\
         %& LM-based@10 & LM-based@10 & 9.58\% & 3.12\% & 0.302\% & 8.68$e^{-2}$\% & 30\% & 40\% & 41.6\% & 33.9\% & 0.712\% & 1.41$e^{-5}$ & 1.21$e^{-7}$ & 8,021,104 \\
         %& LM-based@1 & LM-based@1-INV & 1.05\% & 0.819\% & 5.94$e^{-2}$\% & 4.60$e^{-2}$\% & 0\% & 5\% & 5.4\% & 2.78\% & 1.57\% & 1.29$e^{-6}$ & 4.14$e^{-7}$ & 4,118,358 \\
         %& LM-based@10 & LM-based@1-INV & 2.16\% & 1.86\% & 1.50$e^{-2}$\% & 1.29$e^{-2}$\% & 0\% & 5\% & 4.9\% & 2.7\% & 1.47\% & 1.45$e^{-6}$ & 5.76$e^{-7}$ & 33,298,359\\
         %& LM-based@1 & LM-based@10-INV & 3.92\% & 2.25\% & 0.311\% & 1.76$e^{-1}$\% & 20\% & 17\% & 15.3\% & 9.33\% & 3.10\% & 5.87$e^{-6}$ & 9.76$e^{-7}$ &  2,933,821\\
         & GenT@10 & LM-based@10k-INV & \textbf{7.08\%} & \textbf{4.91\%} & 6.52$e^{-2}$\% & 4.39$e^{-2}$\% & 10\% & 18\% & 15.3\% & 9.29\% & \textbf{3.16\%} & 6.17$e^{-6}$ & \textbf{9.99$e^{-7}$ } & 25,798,594\\
         \hdashline
         & T5-GenT@10 & LM-based@10k-INV & 4.68\% & 2.59\% & 3.32$e^{-2}$\% & 1.77$e^{-2}$\% & XXX & XXX & XXX & 5.24\% & 1.13\% & 3.10$e^{-6}$ & 3.22$e^{-7}$ & 33,874,204 \\
         %& LM-based@1 & LM-based@50-INV & 6.38\% & 1.47\% & 0.601\% & 1.33$e^{-1}$\% & 10\% & 26.0\% & 21.3\% & 15.4\% & 1.97\% &  8.73$e^{-6}$  & 6.06$e^{-7}$ & 2,476,310 \\
         %& LM-based@10 & LM-based@50-INV & \textbf{10.2\%} & 3.20\% & 0.113\% & 3.24$e^{-2}$\% & 20\% & 26\% & 20.5\% & 15.0\% & 1.83\% & 8.07$e^{-6}$  & 6.49$e^{-7}$ & 21,551,772\\
        %Quasimodo & LM-based@1 & LM-based@100-INV & 7.39\% & 0.575\% & 0.733\% & 5.40$e^{-2}$\% & 30\% & 26\% & 21.0\% & 15.3\% & 1.25\% & 8.49$e^{-6}$ & 3.06$e^{-7}$ \\
        %Quasimodo & LM-based@10 & LM-based@100-INV & \textbf{11.8\%} & 1.05\% & 0.137\% & 1.09$e^{-2}$\% & 20\% & 24\% & 18.8\% & 13.9\% & 1.18\% & 8.06$e^{-6}$ & 3.04$e^{-7}$ \\
        %Quasimodo & LM-based@1 & LM-based@25 & 6.64\% & 0.405\% & 4.68\% & 30\% & 39\% & 38.9\% & 33.9\% & 1.41$e^{-5}$  \\
        %Quasimodo & LM-based@10 & LM-based@25 & 9.10\% & 1.64\% & 0.463\% & 30\% & 35\% & 39.8\% & 33.6\% & 1.43$e^{-5}$\\
        %Quasimodo & LM-based@1 & LM-based@50 & 7.89\% & 0.176\% & 10.1\% & 50\% & 40\% & 38.7\% & \textbf{34.0\%} & 1.55$e^{-5}$  \\
        %Quasimodo & LM-based@10 & LM-based@50 & 10.5\% & 1.06\% & 0.813\% & 50\% & 36\% & 39.6\% & 33.3\% & 1.71$e^{-5}$ \\
        %Quasimodo & LM-based@1 & LM-based@100 & 9.04\% & 6.31$e^{-2}$\% & \textbf{16.8\%} & 30\% & 36\% & 35.9\% & 32.8\% & 1.44$e^{-5}$\\
        %Quasimodo & LM-based@10 & LM-based@100 & \textbf{11.9\%} & 0.661\% & 1.50\% & 20\% & 30\% & 35.5\% & 31.5\% & 1.44$e^{-5}$ \\
        %\hdashline
        %Quasimodo & LM-based COMET S & Rule-based & 1.09\% & 0.222\% & 3.72\% & \textbf{100\%} & \textbf{83\%} & 42.2\% & 13.3\% & \textbf{2.59$e^{-5}$}\\
        %Quasimodo & LM-based COMET SP & Rule-based & 2.33\% & 0.803\% & 0.403\% & 30\% & 24\% & 18.6\% & 11.3\% & $8.15e^{-6}$  \\
        %Quasimodo & LM-based COMET S & Rule-based & 0.789\% & 0.174\% & 2.46\% & \textbf{100\%} & 76\% & 36.8\% & 10.3\% & \textbf{2.47$e^{-5}$}\\
        %Quasimodo & LM-based COMET SP & Rule-based & 1.82\% & 0.681\% & 0.314\% & 20\% & 20\% & 21.5\% & 10.2\% & $7.70e^{-6}$  \\
        \hline
        \multirow{8}{*}{Ascent++} & Manual Mapping~\cite{nguyen2021refined} & Manual & 0.468\% & - & 8.83$e^{-2}$\% & - & 0\% & 5\% & 3.2\% & 1.3\% & - & $1.25e^{-6}$  & - & 1,228,001 \\
         & Rule Mining~\cite{soderland2013open,soderland2010adapting,dutta2014semantifying} & Rule-based & 0.364\% & 9.83$e^{-2}$\% & 0.303 & 8.19$e^{-2}$\% & 20\% & 6\% & 2.6\% & 1.6\% & 0.142\% & $4.65e^{-6}$ & 1.22$e^{-7}$ & 277,835\\
         & Classifier~\cite{zhang2019openki} & Rule-based & 1.08\% & 0.294\% & 0.146\% & 4.52$e^{-2}$\% & 20\% & 12\% & 4.3\% & 2.03\% & 8.19$e^{-2}$\% & $2.79e^{-6}$ & 5.58$e^{-8}$ & 1,722,441\\
        \hdashline
         & GenT@1 & Rule-based & 2.78\% & 1.28\% & \textbf{0.493\% } & \textbf{2.25$e^{-1}$\%} & 40\% & 48\% & 20.4\% & 8.52\% & 1.24\% & $1.05e^{-5}$  & 9.89$e^{-7}$ & 1,277,065\\
         & GenT@10 & Rule-based & 4.98\% & 3.15\% & 0.112\% & 6.89$e^{-2}$\% & 50\% & 48\% & 25.1\% & 9.62\% & 1.42\% & $1.42e^{-5}$ & 1.78$e^{-6}$ & 10,193,040\\
        \hdashline
         %& LM-based@1 & LM-based@0.1 & 0.723\% & 0.617\% & 0.137\% & 1.16$e^{-1}$\% & 0\% & 2\% & 1.4\% & 1.33\% & 1.07\% & 4.92$e^{-7}$ & 3.81$^{-7}$ & 1,225,211\\
         %& LM-based@10 & LM-based@0.1 & 2.28\% & 2.10\% & 5.20$e^{-2}$\% & 4.77$e^{-2}$\% & 0\% & 4\% & 2\% & 1.61\% & 1.28\% & 6.91$e^{-7}$  & 5.44$e^{-7}$  & 10,163,805\\
         %& LM-based@1 & LM-based@1 & 2.92\% & 1.70\% & 0.810\% & 4.70$e^{-1}$\% & 60\% & 48\% & 26.6\% & 10.5\% & 3.29\% & 1.54$e^{-5}$ & 7.79$e^{-7}$  & 834,646\\
         & GenT@10 & LM-based@10k & 5.70\% & 4.15\% & 0.191\% & 1.37$e^{-1}$\% & 60\% & 47\% & 25.1\% & \textbf{10.8\%} & 3.43\% & \textbf{1.60$e^{-5}$} & 7.70$e^{-7}$ & 7,000,135 \\
        
         %& LM-based@1 & LM-based@10 & 5.18\% & 1.03\% & \textbf{2.97\%} & \textbf{5.95$e^{-1}$\%} & \textbf{70\%} & \textbf{67\%} & \textbf{53.2\%} & \textbf{31.1\%} & 1.91\% & 2.33$e^{-5}$ & 2.10$e^{-7}$ & 405,114 \\
         %& LM-based@10 & LM-based@10 & 8.27\% & 2.98\% & 0.458\% & 1.54$e^{-1}$\% & \textbf{70\%} & 66\% & 51.8\% & 30.0\% & 1.87\% & \textbf{2.15}$e^{-5}$ & 2.27$e^{-7}$ & 4,346,372 \\
        %Ascent++ & LM-based@1 & LM-based@10 & 6.47\% & 1.04\% & \textbf{2.28\%} & 20\% & 40\% & 40.8\% & 34.5\% & 1.35$e^{-5}$ \\
        %Ascent++ & LM-based@10 & LM-based@10 & 9.58\% & 3.12\% & 0.302\% & 30\% & 40\% & 41.6\% & 33.9\% & 1.41$e^{-5}$ \\
         %& LM-based@1 & LM-based@1-INV & 1.36\% & 1.21\% & 0.283\% & 2.50$e^{-1}$\% & 0\% & 6\% & 4\% & 2.76\% & 2.16\% & 1.50$e^{-6}$ & 8.28$e^{-7}$  & 1,119,032 \\
         %& LM-based@10 & LM-based@1-INV & 5.53\% & 3.28\% & 8.60$e^{-2}$\% & 7.96$e^{-2}$\% & 0\% & 11\% & 5.3\% & 3.41\% & 2.73\% & 3.08$e^{-6}$  & 1.55$e^{-6}$  & 9,544,023 \\
         %& LM-based@1 & LM-based@10-INV & 3.36\% & 1.77\% & 0.790\% & 4.12$e^{-1}$\% & 30\% & 23\% & 16.8\% & 10.4\% & 3.86\% & 9.96$e^{-6}$  & \textbf{2.61$e^{-6}$}  & 986,012 \\
         & GenT@10 & LM-based@10k-INV & \textbf{6.52\%} & \textbf{4.26\%} & 0.184\% & 1.17$e^{-1}$\% & 40\% & 20\% & 18\% & 10.8\% & \textbf{4.15\%} & 9.74$e^{-6}$  & \textbf{1.98$e^{-6}$}  & 8,305,861\\
         %& LM-based@1 & LM-based@50-INV & 5.29\% & 1.05\% & 1.25\% & 2.41$e^{-1}$\% & 20\% & 32\% & 19.3\% & 12.3\% & 1.52\% & 7.99$e^{-6}$  & 5.37$e^{-6}$ & 985,818\\
         %& LM-based@10 & LM-based@50-INV & \textbf{9.18\%} & 2.55\% & 0.262\% & 6.77$e^{-2}$\% & 10\% & 24\% & 17.8\% & 12.0\% & 1.49\% & 6.88$e^{-6}$  & 6.12$e^{-7}$ & 8,257,812\\
        %Ascent++ & LM-based@1 & LM-based@100-INV & 6.18\% & 0.417\% & 1.40\% & 9.21$e^{-2}$\% & 20\% & 23\% & 19.5\% & 11.7\% & 0.937 & 8.03$e^{-6}$  & 4.21$e^{-7}$ \\
        %Ascent++ & LM-based@10 & LM-based@100-INV & \textbf{10.8\%} & 0.883\% & 0.294\% & 2.18$e^{-2}$\% & 10\% & 23\% & 17.9\% & 11.0\% & 0.877\% & 6.96$e^{-6}$  & 4.12$e^{-7}$\\
        
        %Ascent++ & LM-based@1 & Rule-based & 2.38\% & 0.789\% & \underline{\textbf{0.423\%}} & 80\% & 42\% & 18.7\% & 7.4\% & $1.50e^{-5}$ \\
        %Ascent++ & LM-based@10 & Rule-based & \textbf{4.23\%} & \textbf{2.20\%} & 9.77$e^{-2}$\% & \underline{\textbf{90\%}} & \textbf{42\%} & \textbf{21.9\%} & \textbf{8.12\%} & $1.60e^{-5}$\\
        %\hdashline
        %Ascent++ & LM-based COMET S & Rule-based & 0.977\% & 0.358\% & 3.10\% & 100\% & 81\% & 43\% & 12.5\% & $2.63e^{-5}$\\
        %Ascent++ & LM-based COMET SP & Rule-based & 2.15\% & 1.11\% & 0.297\% & 20\% & 25\% & 18.5\% & 1.7\% & $1.11e^{-5}$ \\
        %Ascent++ & LM-based COMET S & Rule-based & 0.772\% & 0.212\% & 2.46\% & 80\% & 62\% & 31.5\% & 9.48\% & $2.24e^{-5}$\\
        %Ascent++ & LM-based COMET SP & Rule-based & 1.74\% & 0.749\% & 0.297\% & 60\% & 20\% & 16.4\% & 8.58\% & $1.12e^{-5}$ \\
        %\hline
        %- & CometKB S & ConceptNet & 1.11\% & 0.144\% & 2.96\% & 20\% & 25\% & 20.1\% & 7.65\% & $6.29e^{-6}$ \\
        %- & CometKB SP & ConceptNet & 2.87\% & 0.504\% & 0.179\% & 10\% & 2\% & 3.2\% & 3.36\% & $1.43e^{-6}$ \\
        %- & CometKB & ConceptNet & 0.641\% & 0.299\% & 9.38$e^{-2}$ & 10\% & 2\% & 1.2\% & 0.27\% \\ 
        \hline
        \multicolumn{15}{c}{Direct Generation} \\
        \hline
        \multirow{4}{*}{Quasimodo} & LM-based COMET S & Rule-based & 1.09\% & 0.222\% & \textbf{3.72\%} & 0.137\% & \textbf{100\%} & \textbf{83\%} & 42.2\% & \textbf{13.3\%} & 1.66\% &\textbf{2.59$e^{-5}$} & 2.96$e^{-7}$ & 67,776 \\
         & GenT COMET SP & Rule-based & 2.33\% & 0.803\% & 0.403\% & 0.782\% & 30\% & 24\% & 18.6\% & 11.3\% & 1.24\% & $8.15e^{-6}$ & 2.66$e^{-7}$ & 1,344,639 \\
        
         & GenT COMET S & LM-based@10k-INV & 0.657\% & 0.285\% & 2.20\% & 0.975\% & 20\% & 17\% & 15.8\% & 7.14\% & 2.86\% & 9.59$e^{-6}$ & 5.20$e^{-6}$ & 69,781 \\
         & GenT COMET SP & LM-based@10k-INV & 1.71\% & 1.07\% & 0.261\% & 0.163\% & 20\% & 21\% & 15.5\% & 6.46\% & 3.12\% & $7.16e^{-6}$ & 3.61$e^{-7}$ & 1,528,633\\
        \hline
        \multirow{4}{*}{Ascent++} & LM-based COMET S & Rule-based & 0.977\% & 0.358\% & 3.10\% & \textbf{1.15\%} & \textbf{100\%} & 81\% & \textbf{43\%} & 12.5\% & 3.90\% & $2.63e^{-5}$ & 2.68$e^{-6}$ & 73,134 \\
         & GenT COMET SP & Rule-based & 2.15\% & \textbf{1.11\%} & 0.345\% & 0.177\% & 100\% & 74\% & 38.7\% & 12.6\% & 4.14\% & $1.11e^{-5}$ & \textbf{6.77$e^{-6}$} & 1,447,597\\
        
         & GenT COMET S & LM-based@10k-INV & 0.825\% & 0.326\% & 2.74\% & 0.326\% & 20\% & 26\% & 28.8\% & 8.94\% & 3.50\% & $6.44e^{-6}$ & 1.26$e^{-6}$ & 70,076 \\
         & GenT COMET SP & LM-based@10k-INV & 2.09\% & 1.10\% & 0.340\% & 0.178\% & 40\% & 24\% & 19.6\% & 10.7\% & \textbf{4.69\%} & $8.74e^{-6}$ & 3.52$e^{-6}$ & 1,431,353 \\
        \hline
        - & Comet S~\cite{comet-atomic-2020} & ConceptNet & 1.11\% & 0.144\% & 2.96\% & 0.401\% & 20\% & 25\% & 20.1\% & 7.65\% & 0.891\% & $6.30e^{-6}$ & 3.04$e^{-7}$ & 87,207 \\
        - & Comet SP~\cite{comet-atomic-2020} & ConceptNet & \textbf{2.87\%} & 0.504\% & 0.179\% & 0.504\% & 10\% & 2\% & 3.2\% & 3.36\% & 0.510 & $1.43e^{-6}$ & 1.28$e^{-7}$ & 1,764,549 \\
        \hline
    \end{tabular}
\end{adjustbox}

    \caption{Automatic Recall And Precision ($^*$ ignores the predicates for OpenKBs).}
    \label{tab:auto_rec_prec}
    \dovspace
\end{table*}

==> parts/tables/jaccard.tex <==
\begin{table}[!ht]
    \centering
\begin{adjustbox}{width=\columnwidth,center}
\begin{tabular}{|c|c|c|c|c|c|c|c|c|c|}
        \hline
        Method & Jaccard & $R_a$ & $\bar{R}_a$ & $P_a$ & $P_a@10$ & $P_a@100$ & $P_a@1000$ & $P_a@10000$ & MRR \\
        \hline
        LM-based@1 & 1.0 & 0.119\% & $6.92e^{-3}$\% & \textbf{0.671\%} & 40\% & 20\% & 7.1\% & 1.52\% & 5.75$e^{-6}$ \\
        LM-based@1 & 0.5 & 1.81\% & 0.320\% & 0.202\% & 60\% & 51\% & 22.6\% & 7.28\% & 1.23$e^{-5}$\\
        LM-based@1 & 0.1 & 2.84\% & 1.03\% & 0.177\% & 80\% & 67\% & 35.7\% & 11.3\% & 1.95$e^{-6}$\\
        LM-based@1 & 0 & 2.94\% & 1.11\% & 0.179 & 80\% & \textbf{78\%} & 39\% & 12.1\% & 2.11$e^{-5}$\\
        \hdashline
        LM-based@10 & 1.0 & 0.186\% & $1.99e^{-2}$\% & 0.196\% & 20\% & 20\% & 6.9\% & 1.6\% & $4.99e^{{-6}}$ \\
        LM-based@10 & 0.5 & 2.81\% & 0.834\% & $5.55e^{-2}$\% & 60\% & 41\% & 21.4\% & 7.64\% & $1.12e^{-5}$ \\
        LM-based@10 & 0.1 & 4.97\% & 2.83\% & $4.18e^{-2}$\% & \textbf{90\%} & 65\% & 36.2\% & 12.5\% & $2.03e^{-6}$\\
        LM-based@10 & 0 & \textbf{5.11\%} & \textbf{2.97\%} & 4.12$e^{-2}$\% & 80\% & 74\% & \textbf{40.2\%} & \textbf{13.5\%} & \textbf{2.16}$e^{-5}$\\
        \hline
    \end{tabular}
\end{adjustbox}

    \caption{Impact of Jaccard Constraints For Quasimodo}
    \label{tab:jaccard}
    \dovspace
\end{table}

==> parts/tables/manual_evaluation.tex <==
\begin{table}[!ht]
    \centering

\begin{adjustbox}{width=\columnwidth,center}
    \input{parts/tables/raw_manual_alignment}
    \input{parts/tables/raw_typicality}
\end{adjustbox}

    \caption{Manual Alignment Evaluation On Quasimodo (left) and Typicality (right).} %\sr{Related-row shows surprisingly low values - what does this exactly capture? Exact semantic match perhaps? That is a stronger requirement, if it is so then the values are fine - then the column should be renamed?}
    \label{tab:all_manual}
    \dovspace
    %\vspace{-10pt}
\end{table}

==> parts/tables/neg_sampling.tex <==
\begin{table}[!ht]
    \centering
\begin{adjustbox}{width=\columnwidth,center}
\begin{tabular}{|c|c|c|c|c|c|c|c|c|c|}
        \hline
        Method & \#Negative & $R_a$ & $\bar{R}_a$ & $P_a$ & $P_a@10$ & $P_a@100$ & $P_a@1000$ & $P_a@10000$ & MRR\\
        \hline
        LM-based@1 & 0 & 2.94\% & 0.979\% & 0.179 & 80\% & \textbf{78\%} & 39\% & 12.11\% & $2.11e^{-5}$ \\
        LM-based@1 & 1k & 2.53\% & 0.779\% & \textbf{0.585\%} & \textbf{90\%} & 68\% & 37.7\% & 12.5\% & $2.13e^{-5}$\\
        LM-based@1 & 10k & 2.55\% & 0.828\% & 0.494\% & 60\% & 65\% & 37.9\% & 12.8\% & $1.92e^{-5}$\\
        LM-based@1 & 100k & 2.20\% & 0.580\% & 0.380\% & 70\% & 62\% & 37.9\% & 12.9\% & $1.82e^{-5}$\\
        \hdashline
        LM-based@10 & 0 & \textbf{5.11\%} & \textbf{2.77\%} & 4.12$e^{-2}$\% & 80\% & 74\% & 40.2\% & 13.5\% & $2.16e^{-5}$ \\
        LM-based@10 & 1k & 4.07\% & 2.00\% & 0.207\% & \textbf{90\%} & 69\% & \textbf{40.3\%} & 14.2\% & \textbf{2.19}$e^{-5}$\\
        LM-based@10 & 10k & 4.15\% & 2.08\% & 0.176\% & 60\% & 71\% & 38.9\% & \textbf{14.3\%} & $1.99e^{-5}$\\
        LM-based@10 & 100k & 3.67\% & 1.68\% & 0.128\% & 70\% & 61\% & 36.8\% & 13.22\% & $1.88e^{-5}$\\
        \hline
    \end{tabular}
\end{adjustbox}

    \caption{Impact of Negative Sampling For Quasimodo}
    \label{tab:neg_sampling}
    \dovspace
\end{table}

==> parts/tables/sizes.tex <==
\begin{table}[!ht]
    \centering

\begin{adjustbox}{width=0.7\columnwidth,center}
\begin{tabular}{|c|c|c|c|c|c|}
        \hline
        KB  & Method & Dataset & Size & Train Size & CF \\
        \hline
        ConceptNet & - & - & 232,532 & - & - \\ 
        \hline
        Quasimodo & - & - & 5,930,628 & - & - \\
        \hdashline
        Quasimodo & Manual Mapping & Manual & 4,925,792 & 0 & 1.00 \\
        Quasimodo & Rule Mining & Rule-based & 689,146 & 33,159 & 2.03 \\
        Quasimodo & Classifier & Rule-based & 5,478,028 & 33,159 & 1.08\\
        \hdashline
        Quasimodo & LM-based@1 & Rule-based & 4,135,349 & 33,159 & 1.43\\
        Quasimodo & LM-based@10 & Rule-based & 33,425,732 & 33,159 & 1.99\\
        %\hdashline
        %Quasimodo & LM-based@10 Jaccard=1.0 & Rule-based & 221,677 & 33,159 & 1.08 \\
        %Quasimodo & LM-based@10 Jaccard=0.5 & Rule-based & 11,897,303 & 33,159 & 1.23 \\
        \hdashline
        %Quasimodo & LM-based@1 & LM-based@0.1 & 2,458,687 & 5,389 & 2.41 \\
        %Quasimodo & LM-based@10 & LM-based@0.1 & 20,738,235 & 5,389 & 2.86 \\
        %Quasimodo & LM-based@1 & LM-based@1 & 1,669,647 & 53,310 & 3.55 \\
        %Quasimodo & LM-based@10 & LM-based@1 & 15,647,853 & 53,310 & 3.79 \\
        %Quasimodo & LM-based@1 & LM-based@10 & 659,120 & 533,713 & 9.00 \\
        Quasimodo & LM-based@10 & LM-based@10 & 8,021,104 & 533,713 & 7.39\\
        %Quasimodo & LM-based@1 & LM-based@1-INV & 4,118,358 & 2,119 & 1.44 \\
        %Quasimodo & LM-based@10 & LM-based@1-INV & 33,298,359 & 2,119 & 1.78\\
        %Quasimodo & LM-based@1 & LM-based@10-INV & 2,933,821 & 20,874 & 2.02 \\
        Quasimodo & LM-based@10 & LM-based@10-INV & 25,798,594 & 20,874 & 2.30\\
        %Quasimodo & LM-based@1 & LM-based@50-INV & 2,476,310 & 104,730 & 2.39 \\
        %Quasimodo & LM-based@10 & LM-based@50-INV & 21,551,772 & 104,730 & 2.75\\
        %Quasimodo & LM-based@1 & LM-based@100-INV & 2,353,294 & 209,397 & 2.52 \\
        %Quasimodo & LM-based@10 & LM-based@100-INV & 20,385,069 & 209,397 & 2.91\\
        %Quasimodo & LM-based@1 & LM-based@25 & 329,885 & 1,334,424 & 18.0\\
        %Quasimodo & LM-based@10 & LM-based@25 & 5,086,008 & 1,334,424 & 11.7 \\
        %Quasimodo & LM-based@1 & LM-based@50 & 181,501 & 2,668,123 & 32.7 \\
        %Quasimodo & LM-based@10 & LM-based@50 & 3,360,898 & 2,668,123 & 17.6 \\
        %Quasimodo & LM-based@1 & LM-based@100 & 125,108 & 5,337,100 & 47.4 \\
        %Quasimodo & LM-based@10 & LM-based@100 & 2,042,975 & 5,337,100 & 29.0 \\
        %\hdashline
        %Quasimodo & LM-based COMET S & Rule-based & 67,776 & 33,159 & 1.29 \\
        %Quasimodo & LM-based COMET SP & Rule-based & 1,344,639 & 33,159 & 1.43 \\
        \hline
        Ascent++ & - & - & 1,967,126 & - & - \\
        \hdashline
        Ascent++ & Manual Mapping & Manual & 1,228,001 & 0 & 1.00 \\
        Ascent++ & Rule Mining & Rule-based & 277,835 & 19,320 & 2.00  \\
        Ascent++ & Classifier & Rule-based & 1,722,441 & 19,320 & 1.14\\
        \hdashline
        Ascent++ & LM-based@1 & Rule-based & 1,277,065 & 19,320  & 1.54 \\
        Ascent++ & LM-based@10 & Rule-based & 10,193,040 & 19,320 & 1.93 \\
        \hdashline
        %Ascent++ & LM-based@1 & LM-based@0.1 & 1,225,211 & 1,739 & 1.61 \\
        %Ascent++ & LM-based@10 & LM-based@0.1 & 10,163,805 & 1.739 & 1.94 \\
        %Ascent++ & LM-based@1 & LM-based@1 & 834,646 & 17,652 & 2.36 \\
        %Ascent++ & LM-based@10 & LM-based@1 & 7,000,135 & 17,652 & 2.81 \\
        %Ascent++ & LM-based@1 & LM-based@10 & 405,114 & 177,041 & 4.86 \\
        Ascent++ & LM-based@10 & LM-based@10 & 4,346,372 & 177,041 & 4.52 \\
        %Ascent++ & LM-based@1 & LM-based@10 & 659,120 & 533,713 & 9.00 \\
        %Ascent++ & LM-based@10 & LM-based@10 & 8,021,104 & 533,713 & 7.39\\
        %Ascent++ & LM-based@1 & LM-based@1-INV & 1,119,032 & 2,088 & 1.76 \\
        %Ascent++ & LM-based@10 & LM-based@1-INV & 9,544,023 & 2,088 & 2.06\\
        %Ascent++ & LM-based@1 & LM-based@10-INV & 986,012 & 20,906 & 2.00 \\
        Ascent++ & LM-based@10 & LM-based@10-INV & 8,305,861 & 20,906 & 2.37\\
        %Ascent++ & LM-based@1 & LM-based@50-INV & 985,818 & 104,615 & 2.00 \\
        %Ascent++ & LM-based@10 & LM-based@50-INV & 8,257,812 & 104,615 & 2.38\\
        %Ascent++ & LM-based@1 & LM-based@100-INV & 1,026,011 & 209,397 & 1.92\\
        %Ascent++ & LM-based@10 & LM-based@100-INV & 8,611,082 & 209,397 & 2.28\\
        %\hdashline
        %Ascent++ & LM-based COMET S & Rule-based & 72,757 & 19,320 & 1.19\\
        %Ascent++ & LM-based COMET SP & Rule-based & 1,359,965 & 19,320  & 1.31 \\
        %\hline
        %- & CometKB S & ConceptNet & 86,978 & 186.025  & 1.0 \\ 
        %- & CometKB SP & ConceptNet & 3,747,155 & 186.025  & 1.04 \\ 
        %- & CometKB & ConceptNet & 1,746,201 & 1.72$e^{-4}$ \\ 
        \hline
    \end{tabular}
\end{adjustbox}

    \caption{Sizes}
    \label{tab:sizes}
    \dovspace
\end{table}
